Integration of physics-informed operator learning and finite element method for parametric learning of partial differential equations

We present a method that employs physics-informed deep learning techniques for parametrically solving partial differential equations. The focus is on the steady-state heat equations within heterogeneous solids exhibiting significant phase contrast. Similar equations manifest in diverse applications like chemical diffusion, electrostatics, and Darcy flow. The neural network aims to establish the link between the complex thermal conductivity profiles and temperature distributions, as well as heat flux components within the microstructure, under fixed boundary conditions. A distinctive aspect is our independence from classical solvers like finite element methods for data. A noteworthy contribution lies in our novel approach to defining the loss function, based on the discretized weak form of the governing equation. This not only reduces the required order of derivatives but also eliminates the need for automatic differentiation in the construction of loss terms, accepting potential numerical errors from the chosen discretization method. As a result, the loss function in this work is an algebraic equation that significantly enhances training efficiency. We benchmark our methodology against the standard finite element method, demonstrating accurate yet faster predictions using the trained neural network for temperature and flux profiles. We also show higher accuracy by using the proposed method compared to purely data-driven approaches for unforeseen scenarios.

==> Extra/draft.tex <==

 
 ´%This current work focuses on the potential of PINN to solve constitutive relations under arbitrary loading scenarios without the need for labeled data. As a result, the costly and repetitive process of nonlinear Newton iterations at the material point level can be omitted 
 %Some authors have employed strategies such as using FFNN with internal variables or RNN to consider the path dependency of the material.

\begin{table}[H]
\centering
\caption{nothing}  
\label{tab:network_cost}
\begin{footnotesize}
\begin{tabular}{ l l }
\hline
Method   &  run-time    \\
\hline
classical algorithm         &   $2.3$  \\ 
COMM-PINN                       &   $1.0$  \\ 
\hline
\end{tabular}
\end{footnotesize}
\end{table}
 
 
 %In the context of material modeling, we need to set up consistent formulations to predict nonlinear material behavior. The latter tasks puzzled the researchers for years. 

%As a result, different material models are developed for each specific application. 

 %As a result, one can guarantee a consistent outcome from the model under any circumstances (i.e. loading process). 


 
%Moreover we discussed ideas to reduce the required order of dervatives for obtaning the tangent operator. 
%and all we need are the constitutive equations for internal variables evolution, and the yield function. 
%\\ \\
%\\ \\
%\textbf{Remark 3} In the current study, the basic material model is derived from dissipation inequality, and all the relevant material physical constraints are already included in the total loss function. Therefore, upon proper training on enough collocation points, the outcome of the network automatically respects the thermodynamical constraints for any arbitrary loading path.

%the fact that losses are satisfied to some extent and still for any unseen collocation point there is no fundamental guarantee in this method. For example, there is no guarantee about the positive definiteness of the obtained stiffness for the case of plasticity with nonlinear isotropic hardening.




%\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\citet{khorrami2022artificial} employed a convolutional neural network to predict the stress fields for history-dependent material behavior. See also \cite{RASHID2022}, where authors employed a Fourier neural operator to predict a stress field at a high resolution by performing the training based on data of low resolution.

%\textcolor{red}{@ali: can u write the formulas for dissipation inequality? just the step before the following relations where we set the parenthesis to zero.}

%Applying the second-law of thermodynamics in terms of the Clausius-Duhem inequality, consistent state relations of the model are derived. 

In this work, the hyperbolic-tangent function is utilized which is defined as
\begin{equation}
\label{eq:af}
    \tanh(x)=\dfrac{\exp^x - \exp^{-x}}{\exp^x + \exp^{-x}}. 
\end{equation}


\begin{align}
\label{eq:CDI}
   -\dot{\psi} + \sigma~\dot{\epsilon} \stackrel{!}{\ge} 0.
\end{align}


%%% Sequential training swish 
\subsection{Sequential training for \emph{swish}}
Losses for the sequential training 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/seq_swish_losses.jpg}
  \caption{Losses for the sequential training, mechanics and thermal losses, swish as activation function}
  \label{fig:losses_seq_swish}
\end{figure}
Total loss
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/seq_swish_total_loss.jpg}
  \caption{Total losses for the sequential training, mechanics and thermal total losses, swish}
  \label{fig:total_loss_seq_swish}
\end{figure}
Deformed figures 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/seq_deform_swish}
  \caption{Deformed state of boundary value problem for the sequential training, swish}
  \label{fig:defo_seq_swish}
\end{figure}
Results for the mechanical field 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/mechanic_seq_swish_3_20.pdf}
  \caption{Obtained results for thermal elasticity problem employing sequential training, mechanical field, swish }
  \label{fig:mech_seq_swish}
\end{figure}
Results for the thermal field field 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/temperature_seq_swish_3_20.pdf}
  \caption{Obtained results for thermal elasticity problem employing sequential training, thermal field, swish }
  \label{fig:tem_seq_swish}
\end{figure}
Coupled Swish
%%% Coupled training swish 
\subsection{Coupled training for \emph{swish}}
Losses for the coupled training 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/cop_swish_losses.jpg}
  \caption{Losses for the coupled training, swish as activation function}
  \label{fig:losses_cop_swish}
\end{figure}
Total loss
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/cop_swish_total_loss.jpg}
  \caption{Total losses for the coupled training, mechanics and thermal total losses, swish}
  \label{fig:total_loss_cop_swish}
\end{figure}
Deformed figures 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/cop_deform_swish}
  \caption{Deformed state of boundary value problem for the sequential training, swish}
  \label{fig:defo_cop_swish}
\end{figure}
Results for the mechanical field 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/mechanic_cop_swish_3_20.pdf}
  \caption{Obtained results for thermal elasticity problem employing sequential training, mechanical field, swish }
  \label{fig:mech_cop_swish}
\end{figure}
Results for the thermal field field 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/temperature_cop_swish_3_20.pdf}
  \caption{Obtained results for thermal elasticity problem employing sequential training, thermal field, swish }
  \label{fig:tem_cop_swish}
\end{figure}


%The solution to the mechanical problem is calculated by minimizing the total loss function in Eq.~\ref{Totalloss} on the set of collocation points. The final optimization reads as:


%In this work, the Adam optimizer \cite{kingma2014adam} is employed. Several parameters and hyper-parameters affect the network’s performance, such as activation function, learning rate, number of epochs, batch size, number of hidden layers, and number of neurons in each layer. Their influence should be investigated based on the number of collocation points and the network’s architecture. This matter is explained in more detail in Section \ref{sec:hype}.

%The architecture of the network for the mechanical problem is shown in Fig.~\ref{fig:PINNs_net_m}. The network is based on the Eqs.~\ref{Totalloss} to \ref{loss_NBCx} which shows up on the right-hand side of the figure. The proposed network in this study shares some similarities with the recent and previous investigation in the literature \cite{Henkes2022, SAMANIEGO2020112790, FUHG2022110839, HAGHIGHAT2021, RAISSI2019}. Nevertheless, it also differs from them in the following aspects. First, the network takes components of the position vector as inputs ($x$ and $y$ coordinate in a 2D setting) and predicts the components of the deformation vector $\bm{u}$ and stress tensor $\bm{\sigma}^O$ as outputs. 
%Using the predicted deformation vector components ($u_x$ and $u_y$) and based on the kinematic relation (Eq.~\ref{kinematics}) and constitutive law (Eq.~\ref{materiallaw4}), strain and stress tensors are calculated from automatic differentiation, respectively. The latter quantities are denoted by $\bm{\varepsilon}$ and $\bm{\sigma}$. This stress tensor is evaluated from deformation $\bm{u}$ and it is in principle different from the stress tensor $\bm{\sigma}^O$ which is the direct output of the network. Later on, these quantities are forced to take the same value utilizing the connection loss term $\mathcal{L}_{cnc}$ presented in Eq.~\ref{loss_cnc}. Next, in the new design, we consider separate networks for each of the output variables. According to our investigations which will be reported later on in this work, having separated networks for each output quantity shows some advantages compared to the case where all the networks are combined. 


\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/section_geo2_y_5.pdf}
  \caption{Comparison of main outputs of the networks through the section at $y=0.5 \text{mm}$ of the second geometry.}
  \label{fig:sectiongeo2y}
\end{figure}
\newpage

%\begin{figure}[H] 
%  \centering
%  \includegraphics[width=0.9\linewidth]{%./Figs/losses_geo1_cup.pdf}
%  \caption{Prominent loss terms for the %mechanical field decay during the %training procedure utilizing the coupled %training algorithm.}
%  \label{fig:lossesM_cop_tanh_5_40}
%\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/deform_seq_geo1.pdf}
  \caption{Left: undeformed configuration of evaluation points in PINNs. Middle: deformed configuration of evaluation points in PINNs employing sequential training. Right: deformed configuration of the discretized domain in FE analysis. \textcolor{blue}{@Ahmad can you please makes the text and ticks with a bigger fonts}}
  \label{fig:defo_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/mechanic_seq_geo1.pdf}
  \caption{The mechanical field results of the thermoelasticity problem employing the sequential training procedure. Left: PINNs, Middle: FEM, Right: FEM with PINNs difference.}
  \label{fig:mech_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/temperature_seq_geo1.pdf}
  \caption{The thermal field results of the thermoelasticity problem employing the sequential training procedure. Left: PINNs, Middle: FEM, Right: FEM with PINNs difference.}
  \label{fig:tem_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/section_geo1_y_5.pdf}
  \caption{Comparison of main outputs of the networks through the section at $x=0.5 \text{mm}$. Mix. PINNs: denotes to the formulation of this paper by having the $\bm{\sigma}$ and $\bm{u}$ as outputs and utilizing the energy form loss in addition to conventional losses. PINNs: stands for the standard same formulation which has only $\bm{u}$ as output in the absence of the energy form of the problem in the loss function. Couple: minimizing loss function utilizing coupled training algorithm. Sequential: minimization is done with the proposed sequential training method.
  \textcolor{blue}{@Ahmad can you please makes the text and ticks with a bigger fonts and one suggestion Please keep the color and linestyle for FE, use blue color for both mixed pinns red for PINNs then -- for sequential and .. for coupled}}
  \label{fig:sectiongeo1y}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/deform_seq_geo2.pdf}
  \caption{Undeformed and deformed configurations result from the mixed PINNs formulation employing sequential training algorithm and FEM respecting the second geometry. No magnification is made.}
  \label{fig:defo_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/mechanic_seq_geo2.pdf}
  \caption{The mechanical field results of the thermoelasticity for the second geometry using sequential training. Left: PINNs, Middle: FEM, Right: FEM with PINNs difference.}
  \label{fig:mech_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/temperature_seq_geo2.pdf}
  \caption{The thermal field results of the thermoelasticity for the second geometry using sequential training. Left: PINNs, Middle: FEM, Right: FEM with PINNs difference.}
  \label{fig:tem_seq_tanh_5_40}
\end{figure}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.9\linewidth]{./Figs/section_tl_E12_yy.pdf}
  \caption{Comparison of main outputs of the networks through the section at $y=0.5 \text{mm}$ of the second geometry using mixed PINNs formulation combined with data utilizing transfer learning training procedure or pure data-driven scheme.\textcolor{blue}{@Ahmad please also take previous section comments here}}
  \label{fig:sectiongeo2_TL}
\end{figure}

%\begin{align}
%\label{loss_weak}
%\mathcal{L}^{EF}_M &= \text{MAE}^{EF}_M\left(\int_{\Omega}\dfrac{1}{2}\hat{\bm{\varepsilon}}^T\,\hat{{{C}}}(x,y)\,\hat{\bm{\varepsilon}\,~dV - 
%\int_{\Omega}\dfrac{1}{2}\alpha(x,y)\left(T-T_0\right)\,\hat{{{C}}}(x,y)\,\hat{\bm{\varepsilon}}\,~dV}-
%\int_{\Gamma_N} {\bm{u}^T}\,\bar{\bm{t}}~dA\right), \\
%\label{loss_DBC}
%\mathcal{L}^{DBC}_M &= \text{MSE}^{DBC}_M\left( \bm{u} - \overline{\bm{u}} \right), \\
%\label{loss_cnc}
%\mathcal{L}^{cnc}_M &= \text{MSE}^{cnc}_M\left( \bm{\sigma}^o - \bm{\sigma} \right), \\
%\label{loss_SF}
%\mathcal{L}^{SF}_M &= \text{MSE}^{SF}_M\left( \text{div}(\bm{\sigma}^o) \right), \\
%\label{loss_NBCx}  
%\mathcal{L}^{NBC}_M &= \text{MSE}^{NBC}_M\left(\bm{\sigma}^o \cdot \bm{n} - \overline{\bm{t}} \right).
%\end{align}

\dfrac{1}{N^T_{NBC}} \sum_{\bm{X}\in \Gamma^T_N}
\left(\mathcal{N}_{\sigma^o_{xy}}-0\right)^2 
+ \dfrac{1}{N^B_{NBC}} \sum_{\bm{X}\in \Gamma^B_N} ^2
\left(\mathcal{N}_{\sigma^o_{xy}}-0\right)^2 
 \\
&+ \dfrac{1}{N^R_{NBC}} \sum_{\bm{X}\in \Gamma^R_N} \left(\mathcal{N}_{\sigma^o_{xy}}-0\right)^2 +  \dfrac{1}{N^L_{NBC}} \sum_{\bm{X}\in \Gamma^L_N} \left(\mathcal{N}_{\sigma^o_{xy}}-0\right)^2.

% I have removed since we dont have the data falei again
%After considering all of the available sets of ratio values, the training ends. For the pure data-driven case (employing no physical constraints), the big data set is built for all of the cases and the hyperparameters of the network are optimized concerning all of the cases simultaneously. It is worth mentioning that the final number of epochs will be the same for both cases. 

%The ability of the network to predict the response of a given boundary value problem is addressed by looking into a new ratio value $E_r=K_r=15$ (that does not exist in the training data sets).  The corresponding result for the mechanical and thermal fields are plotted in 
%Fig.\,\ref{fig:TL_mixed_pinn_mechanical}, and Fig.\,\ref{fig:TL_mixed_pinn_thermal} by utilizing data and physics.


%\begin{figure}[H] 
%  \centering
%  \includegraphics[width=0.9\linewidth]{./Figs/%E_15t__newmix_0_1.pdf}
%  \caption{The thermal field results of the %thermoelasticity for the case of $E_r=K_r=15$. %Left: PINNs (employing physics and data %($w=0.1$)), Middle: FEM, Right: FEM with PINNs %difference.}
%  \label{fig:TL_mixed_pinn_thermal}
%\end{figure}

%\begin{figure}[H] 
%  \centering
%  \includegraphics[width=0.9\linewidth]{./Figs/%E_15t_puredata_falei.pdf}
%  \caption{The thermal field results of the %thermoelasticity for the case of $E_r=K_r=15$. %Left: data-driven, Middle: FEM, Right: FEM with %a data-driven difference.}
%  \label{fig:TL_data_thermal}
%\end{figure} 

%The temperature field-related outputs evaluated by PINNs and FEM are depicted in Fig.\,\ref{fig:tem_seq_tanh_5_40}. 

% Moreover, Fig.\,\ref{fig:mech_seq_tanh_5_40} shows also some sort of error on the top and bottom edges for the $u_y$ components which differs from the coupled training.


==> Extra/loading_path.tex <==
\section{Generation of loading paths and relative collocation points}
The location of collocation points plays a crucial role in successful training \cite{REZAEI2022PINN}. Note that \textit{collocation points} include initial inputs for which the governing equations are going to be satisfied (collected). Therefore in principle, they can be different than \textit{data points} for which we know the solution in advance. 
The input of the NN is the given strain at step $i+1$ (i.e. $\epsilon^{i+1}$) as well as state variables from the previous time step $i$ (i.e. $\epsilon^{i}_p$ and $\xi^{i}$). For the given strain (or gap), one can create a random set of loading paths. Here, we divide the time frame into $TF$ number of points which stands for times frames. For the loading, we choose $CP$ number of points which stands for control points. At this point, we have a grid area by defining these points along the time and strain axis. By connecting these grid points via simple linear interpolation as shown in Fig.~\ref{fig:load_path}, we obtain loading paths. For the current studies, we always start at the state of zero stain/gap at time $t=0$ and we also end the loading at time $t=1$ by setting the strain/gap to zero again.
Following the suggested pattern, we end up with $CP^{TF}$ unique loading paths. Each of these paths shall result into a unique stress response in time. 
\begin{figure}[H] 
  \centering
  \includegraphics[width=0.8\linewidth]{./Figs/loading_paths.jpg}
  \caption{Loading paths to obtained the collocation points. A sample loading scenario is shown in dashed line.}
  \label{fig:load_path}
\end{figure}
Next, each loading path is discretized in (pseudo) time via time step size $\Delta t$. The time step size is fixed in the current study. Finally, we require to have some valid values for the second and third input of the NN (i.e. $\epsilon^{i}_p$ and $\xi^{i}$). At this point, one can simply assign some random values to these two quantities as long as they are meaningful for the response of the desired material model. For example the accumulative plastic strain is always bigger than the plastic strain value. Since checking all these constraints might be a bit tricky, we decided to run the numerical material model on the given loading paths and save the results for further training. In this way we make sure that the given inputs to the NN are all admissible values based on a valid consistent model. Nevertheless, as mentioned, one is not limited to this method and can freely choose other random (yet valid) values. Note that only the values of the previous time step is under focus and do not necessarily want to use the solution. Considering the specific case shown in Fig.~\ref{fig:load_path} and $\Delta t = 0.01$, we end up with $CP^{TF}/\Delta t = 7^4~(1/100) = 240100$ sets of collocation points for the training. Each set contains $3$ values for $\epsilon^{i+1}$, $\epsilon^{i}_p$ and $\xi^{i}$.

==> draft.tex <==
%\begin{align}
%\frac{\partial N_1}{\partial \xi} &= -\frac{1}{4}(1 - \eta), & \frac{\partial N_1}{\partial \eta} &= -\frac{1}{4}(1 - \xi), \
%\frac{\partial N_2}{\partial \xi} &= \frac{1}{4}(1 - \eta), & \frac{\partial N_2}{\partial \eta} &= -\frac{1}{4}(1 + \xi), \
%\frac{\partial N_3}{\partial \xi} &= \frac{1}{4}(1 + \eta), & \frac{\partial N_3}{\partial \eta} &= \frac{1}{4}(1 + \xi), \
%\frac{\partial N_4}{\partial \xi} &= -\frac{1}{4}(1 + \eta), & \frac{\partial N_4}{\partial \eta} &= \frac{1}{4}(1 - \xi).
%\end{align}

% 
%Next, we review the finite element implementation of the model. The weak form is constructed by multiplying the equations in Eq. \ref{eq:strong form govering equations}(a-c) by a corresponding arbitrary test function and integrating them over the domain of the problem. With integration by parts, the corresponding weak forms are:
%\begin{align}
%\int_{\Omega}k\nabla T \nabla \delta_{T}dV -\int_{\Omega_t}k\nabla T \delta_{T}dS +\int_{\Omega}\rho {c}\dot{T}\delta_{T}dV-\int_{\Omega}Q\delta_{T}dV=0.
%\end{align} 
%\label{eq:weak_form}

\begin{figure}[H] 
  \centering
  \includegraphics[width=0.99\linewidth]{./Figs/NN_FE.jpg}
  \caption{ Network architecture and loss functions for the COMM-PINN applied to interface failure with nonlinear softening law. }
  \label{fig:NN_FE}
\end{figure}

%\begin{align}
%\label{eq:dis_residual}
%\boldsymbol r_{T}=&\int_{\Omega} [\boldsymbol  B_{T}]^T k\boldsymbol  B_{T} dV-\int_{\Omega_t}[\boldsymbol  B_{T}]^T k\boldsymbol  N_{T}dS +\int_{\Omega}\rho c \dot T [\boldsymbol  N_{T}]dV-\int_{\Omega} [\boldsymbol  N_{T}]^TQdV. 
%\end{align}

\begin{algorithm}[H]
\caption{Solving the damage governing equations at pseudo time $t^{i+1}$}
\label{alg:dmg}
\begin{algorithmic}[1]
\item[\textbf{Input:}] interface's parameters, current gap: ${g}^{i+1}$, history variables: $d^i$, $\xi^i_d$
\item[\textbf{Output:}] current traction: ${T}^{i+1}$, current history variables $d^{i+1}$, $\xi_d^{i+1}$, tangent: ${C}_d=\text{d} {T}^{i+1} / \text{d} {g}^{i+1}$
\State $k=1$
\State Set trial values: ${g}^k_p={g}^{i}_p$, $d^k=\xi^{i}_d=d^i$
\State \textbf{loop} \textit{damage solver} \textbf{do} \\
\vspace{1mm}
$\qquad $ \textbf{if} $\phi^{tr}_d = {K} (g^{i+1})^2 - \left( Y_{0} + q_d(\xi^{i}) \right) \le 0$ \\
\vspace{1mm}
$\qquad $ $\qquad $   $d^{i+1}=d^{i}$, $\xi^{i+1}_d=\xi^{i}_d$ and ${C}_d=(1-d^{i+1})^2K $ \\ 
\vspace{1mm}
$\qquad $ \textbf{else} solve for $d^{k+1}$ and $\xi^{k+1}_d = \xi^{i}_d+\Delta \lambda^{k+1}_d$ (see Eqs~\ref{eq:dm_y},\ref{eq:dmg_ev})\\
\vspace{1mm}
$\qquad $  $\qquad  r^{(1)}_d = d^{k+1} - d^i - (\xi^{k+1}_d - \xi^{i}_d) \dfrac{\partial \phi_d}{\partial Y} \stackrel{!}{=} 0$ \\
$\qquad $  $\qquad  r^{(2)}_d = \phi_d = Y - \left( Y_{0} + q_d\left( \xi^{i+1}_d \right) \right) \stackrel{!}{=} 0$ \\
\vspace{1mm}
$\qquad$  $\qquad [d^{i+1,k+1}~~~ \xi^{i+1,k+1}_d]^T = [d^{i+1,k}~~~\xi^{i+1,k}_d]^T - \boldsymbol{K}_d^{-1} \boldsymbol{r}_d$ \\
%$\qquad $  $\qquad  $ Update the values of $d^{k+1}$, $\xi^{k+1}_d$ \\
$\qquad $ \textbf{end if} \\
\vspace{1mm}
$\qquad $ \textbf{if} $\left| {d}^{i+1,k+1}-{d}^{i+1,k}\right|>\text{tol} $ \textbf{OR} $\left| \xi^{i+1,k+1}_d-\xi^{i+1,k}_d\right|>\text{tol}$ \\
$\qquad $ $\qquad $   $k++$ \\
$\qquad $ $\qquad $   \textbf{CYCLE loop} \textit{damage solver} \\ 
$\qquad $ \textbf{else} \\
$\qquad $ $\qquad $  $d^{i+1}=d^{i+1,k+1}$, $\xi^{i+1}_d=\xi^{i+1,k+1}_d$ \\
\vspace{1mm}
$\qquad $ $\qquad $   \textbf{EXIT loop} \textit{damage solver} \\
$\qquad $ \textbf{end if}
\vspace{1mm}
\State \textbf{end loop}
\State Compute traction ${T}=(1-d^{i+1})^2 {K} {g}^{i+1}$
\State Compute tangent ${C}_d $ 
\end{algorithmic}
\end{algorithm}

\begin{align}
N_1 = \frac{1}{4} (1 - \xi) (1 - \eta),~
N_2= \frac{1}{4} (1 + \xi) (1 - \eta),~
N_3 = \frac{1}{4} (1 + \xi) (1 + \eta),~
N_4 = \frac{1}{4} (1 - \xi) (1 + \eta)
\end{align}


\begin{align}
\label{loss_ene}
\mathcal{L}_{ene} &= \text{MSE}\left( (d^{i+1}-d^{i})\text{Relu}(-\phi^{tr}_d) \right), \\
\label{loss_bcs}
\mathcal{L}_{dbc} &= \text{MSE}\left( (\xi^{i+1}_d-\xi^{i}_d)\text{Relu}(-\phi^{tr}_d) \right).
\end{align}

The mean squared error is defined as
\begin{align}
\label{eq:MSE}
\text{MSE}( \bullet )_{type} &= \dfrac{1}{n}\sum_{i=1}^{n}(\bullet)^2, 
\end{align}
where $n$ is the number of observation points. 




\begin{align}
\label{Totalloss}
\mathcal{L}_{tot} =  
\underbrace{
\sum_{e=1}^{n_{el}}\boldsymbol T^T_e \left[ \boldsymbol \sum_{n=1}^{n_{int}} \dfrac{w_n}{2}~\text{det}(\boldsymbol J)~\boldsymbol B_{T}^T [\boldsymbol C_e] \boldsymbol B_{T} \right] \boldsymbol T_e 
}_{\text{energy + Neumann BCs}} 
+
\quad \lambda_b\underbrace{\sum_{i=1}^{n_{db}} \mathcal{L}_{db,i}}_{\text{Drichlet BCs}} 
\end{align}


The creation of sample are described in Alg.~\ref{alg:sample}.
\begin{algorithm}[H]
\caption{Collocation point generation for solving the interface damage model}
\label{alg:sample}
\begin{algorithmic}[1]
\item[\textbf{Input:}] step size: $st$, begin $bg$ and end of interval $en$, $n=1$
\item[\textbf{Output:}] admissible set of inputs for training $\bold{IN}_d$
\State Initializing: $\boldsymbol{g}=[bg_{g}:st_{g}:en_{g}]$, $\boldsymbol{d}=[bg_{d}:st_{d}:en_{d}]$, $\boldsymbol{\xi}_d=[bg_{\xi_d}:st_{\xi_d}:en_{\xi_d}]$
\State \textbf{for} l \textbf{in} $\boldsymbol{g}$ \textbf{do} \\
\vspace{1mm}
$\qquad $ \textbf{for} j \textbf{in} $\boldsymbol{d}$ \textbf{do} \\
\vspace{1mm}
$\qquad $ $\qquad $ \textbf{for} k \textbf{in} $\boldsymbol{\xi_d}$ \textbf{do} \\ 
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad $ $\bold{IN}_d[n,1]$ = $\boldsymbol{g}[l]$\\
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad $ $\bold{IN}_d[n,2]$ = $\boldsymbol{d}[j]$\\
\vspace{1mm}
$\qquad$ $\qquad$ $\qquad$ \textbf{if} $\boldsymbol{\xi}_d[k] = \boldsymbol{d}[j]$  \\
\vspace{1mm}
$\qquad $ $\qquad$ $\qquad$ $\qquad$ $\bold{IN}_d[n,3]$ = $\boldsymbol{\xi}_d[k]$\\
\vspace{1mm}
$\qquad $ $\qquad $ $\qquad$ $\qquad$ $n++$\\
$\qquad $ $\qquad $ $\qquad$ \textbf{end if}
\end{algorithmic}
\end{algorithm}
